Topics in the phenomenology of axions: the cases of cosmic strings and superradiance

Originally proposed as a solution to the strong CP problem and later understood to be a good dark matter candidates, axions have appeared in a variety of beyond-the-standard-model theories and are imbued with rich phenomelogical consequences. In this dissertation, we will examine two of these consequences: the emission of axions from cosmic strings and the superradiant mechanism in black hole physics. The spontaneous symmetry breaking of a global symmetry in the early universe can give rise to a network of cosmic strings, which emit ultra light, axion-like particles that can contribute to the dark matter density. We will discuss how the associated density fluctuations of these particles can be computed from first principles by treating them as a collection of plane waves. We will then calculate the density power spectrum and compare it to well-established cosmological observables, as well as to observables from future surveys, to derive constraints on the mass of the particles and the symmetry breaking scale. These light axion-like particles can also form a gravitational atom around a spinning black hole through the superradiance process. Considering the black hole to be part of a binary system, the tidal potential of the companion periodically perturbs the gravitational atom such that an atomic transition occurs between two of its energy states. Gravitational waves are emitted by the cloud during this transition. We will derive the analytical formulae of both the strain waveform and frequency spectrum of the signal and identify the systems that would be the most promising for detecting it in future, space-based gravitational wave observatories.

==> abbreviations.tex <==
\singlespacing
\begin{tabular}{l p{5in}} 
%if the terms in the first column are longer than 1.4 inches reduce the number 5 appropriately
A.  QCD & Quantum chromodynamics\\
\\
B.  CP & Charge and parity\\
\\
C.  PQ & Peccei-Quinn\\
\\%This adds the single space between definitions (required)
D.  ALP & Axion-like particles\\
\\
E.  WKB & Wentzel–Kramers–Brillouin \\
\\
F.  CDM & Cold dark matter \\
\\
G.  UV & Ultra-violet \\ 
\\
H.  UVLF & Ultra-violet luminosity function \\
\\
I.  SDSS & Sloan digital sky survey \\
\\
J.  CMB & Cosmic microwave background \\ 
\\
K.  STFT & Short time fourier transform \\
\\
L.  GA & Gravitational atom \\
\\
M.  SNR & Signal to noise ratio \\
\\
N.  GW & Gravitational wave \\
\\
O.  TT & Transverse and rraceless \\
\\
P.  LIGO & Laser interferometer gravitational wave observatory
\\
\\
Q.  LISA & Laser interferometer space antenna \\
\\
R.  DECIGO & Deci-Hz interferometer gravitational wave observatory

\end{tabular}
\doublespacing


==> abstractFile.tex <==
Originally proposed as a solution to the strong CP problem and later understood to be a good dark matter candidates, axions have appeared in a variety of beyond-the-standard-model theories and are imbued with rich phenomelogical consequences. In this dissertation, we will examine two of these consequences: the emission of axions from cosmic strings and the superradiant mechanism in black hole physics. 

The spontaneous symmetry breaking of a global symmetry in the early universe can give rise to a network of cosmic strings, which emit ultra light, axion-like particles that can contribute to the dark matter density. We will discuss how the associated density fluctuations of these particles can be computed from first principles by treating them as a collection of plane waves. We will then calculate the density power spectrum and compare it to well-established cosmological observables, as well as to observables from future surveys, to derive constraints on the mass of the particles and the symmetry breaking scale.   

These light axion-like particles can also form a gravitational atom around a spinning black hole
through the superradiance process. Considering the black hole to be part of a binary system,
the tidal potential of the companion periodically perturbs the gravitational atom such that an atomic
transition occurs between two of its energy states. Gravitational waves are emitted by the cloud during this transition. We will derive
the analytical formulae of both the strain waveform and frequency spectrum of the signal and identify the systems that would be the most promising for detecting it in future, space-based gravitational wave observatories. 

==> acknowledgementsFile.tex <==
I do not think that I would have successfully traveled down the PhD road without the help, support and encouragement of my advisor, Pierre Sikivie. If I have learned anything about what it means to be a scientist and an academic, I owe that to him. \\
I would also like to thank all my teachers and collaborators at the University of Florida that have contributed to my scientific education, each one in their own way: Professors Jeff Dror, Wei Xue, Richard Woodard, Dr. Fengwei Yang and my office mate and fellow graduate student Yuxin Zhao. \\
The Onassis foundation supported me financially from 2023 to 2025; their funding allowed me to take my mind off the financial strains that burden most graduate students and dedicate as much time as possible to my research. I am grateful to them for believing in me. I would also like to thank the Physics department of the University of Florida for awarding me the Steigleman Family Fellowship.
\\ 
It would be a grave omission on my part if I did not take the opportunity to thank all the wonderful friends I have made in Gainesville over the five years that I have lived here: Simon Taipliadis, Armin Niknam, Anthony Smith, Panagiotis Kotoulas, Yiannis Michaloliakos, Rebika Makaju, Brinden (Bear) Carlson, Karthik Srinivasan, Matthew Reinhard, David Sadek, Pranav Satheesh, Soumitra Ganguly, Davis Chen, Brooke Emison, Eva Garcia Ferres, Sikhander Khare, Abhay Alaukik, Chris Litos and many others. I am grateful to all of them for the wonderful times.  

 I try to avoid cliches as much as possible, but I do have to thank my parents and family for all their support and help throughout this PhD degree and well before that. 

Lastly, I have to thank Eleni Papadopoulou for a number of things that would take up this entire dissertation, but most importantly, I have to thank her for making my days unpredictable, whimsical and a lot more bearable. 
 

==> biographyFile.tex <==
Antonios Kyriazis was born in Naoussa, Imathias of Central Macedonia in Greece. He moved to Heraklion, Crete in 2016 to pursue a Bachelor's degree in physics, which he completed in the summer of 2020 at the top of his class. In January of 2021, he joined the physics department at the University of Florida to pursue a PhD in physics. He joined Pierre Sikivie's group in the summer of that year and completed his studies in the summer of 2026. The physics department of the University of Florida awarded him the Charles F. Hooper Jr. Memorial Award and the Steigleman Family Fellowship for his research, while he was also financially supported partly by the Onassis foundation in the years 2023-2025.    

==> dedicationFile.tex <==
To those who hustle each and every day, for a piece of shadow under the flaming sun.
